DSPy Assertions: Computational Constraints for Self-Refining Language Model Pipelines

Chaining language model (LM) calls as composable modules is fueling a new way of programming, but ensuring LMs adhere to important constraints requires heuristic "prompt engineering". We introduce LM Assertions, a programming construct for expressing computational constraints that LMs should satisfy. We integrate our constructs into the recent DSPy programming model for LMs, and present new strategies that allow DSPy to compile programs with LM Assertions into more reliable and accurate systems. We also propose strategies to use assertions at inference time for automatic self-refinement with LMs. We report on four diverse case studies for text generation and find that LM Assertions improve not only compliance with imposed rules but also downstream task performance, passing constraints up to 164% more often and generating up to 37% more higher-quality responses. Our reference implementation of LM Assertions is integrated into DSPy at https://github.com/stanfordnlp/dspy

==> evaluation-hotpot.tex <==
\subsection{Case Study: Multi-Hop QA}
\label{sec:eval-hotpot}

\subsubsection{Task \& Metrics} \label{MultiHopQA_Task_Metrics}

In this task, we explore complex question answering through the multi-hop program from \citet{khattab2023dspy}. This task involves generating queries related to the given question, iteratively retrieving relevant context from a search index, and synthesizing this information to generate an answer. 

\Cref{fig:hotpotqa} shows an implementation of this task in DSPy. 
As shown, in each hop, a \code{dspy.ChainOfThought} module generates a search query for the retriever based on the current accumulated context and the initial question. A \code{dspy.Retrieve} then fetches $k$ relevant passages which are aggregated to the context. Once the loop reaches the maximum number of hops, a \code{dspy.ChainOfThought} module produces the final answer.
With this task and LM pipeline, we aim to produce a robust and thorough reasoning process leading to accurate answers to questions.

We assess intrinsic performance using a Suggestions Passed metric, which quantifies the proportion of suggestions passed across at inference time. For programs with LM Assertions, we measure the last run of the backtracking process (if any).
For extrinsic quality, we use (1) Retrieval Score, which quantifies the proportion of correctly retrieved  \str{gold} passages, and (2) Answer Correctness, which checks if the generated answer precisely matches the \str{gold} standard answer. Both of these are not possible to use directly at inference time, since they require access to ground-truth labels.



\subsubsection{Constraints Specified} \todo{move to appendix}

We define two simple @Suggest@ statements. First, we suggest that the query generated be short and less than 100 characters, with the goal of reducing imprecise retrieval.
Second, we require that a generated query is distinct from previous queries. This discourages the pipeline from retrieving redundant context in each hop.
Note that the condition checks for both constraints are implemented using simple Python code.
Overall, these constraints enable the self-refinement of the search queries generated by the program.

\subsubsection{Evaluation} \label{MultiHopQA_Evaluation}  \todo{move to appendix and replace with focused evaluation description on best numbers with assertions}


For this task, we evaluate the MultiHopQA program under various configurations to understand the impact of LM Assertions and few-shot learning techniques. \Cref{tab:hotpotqa-combined-eval} shows the results of this evaluation.

\todo{update with latest numbers}

Our simplest baseline is the MultiHopQA in a zero-shot, uncompiled configuration (\str{ZeroShot}--\str{NoSuggest}). When we include the mentioned assertions within this zero-shot configuration (\str{ZeroShot}--\str{Suggest}), we see a notable improvement of $35.7\%$ more suggestions passed, meaning the retrieval query generation LM is more likely to generate concise, precise, and distinct queries.
Then, we observe $\approx$13.3\% in the retrieval score and an indirect $\approx$1.3\% increase in answer correctness due to refined query generation.

\todo{mention the new fewshot configurations comparisons}
We take advantage of optimizations in the DSPy compiling framework, utilizing the \code{BootstrapFewShotWithRandomSearch} teleprompter, which automatically generates and integrates few-shot examples doing a random search over a set of candidates within the MultiHopQA program. We include a maximum of 2 bootstrapped few-shot examples to fit within the context window and compile 6 candidates on the devset examples.
We apply this evaluation approach to both the vanilla MultiHopQA and the MultiHopQA with Assertions programs. In the non-assertion configuration (\str{FewShot}--\str{NoSuggest}), we see a strong performance gain in retrieval score and correctness, which highlights the efficacy of utilizing few-shot techniques to refine the querying and reasoning processes. We find that combining few-shot learning with assertions (\str{FewShot}--\str{Suggest}) further demonstrates improvements of both $\approx$27.2\% more passed constraints and $\approx$1.4--4.2\% on both extrinsic metrics.








